Strategic Port Graph Rewriting: An Interactive Modelling and Analysis Framework

We present strategic portgraph rewriting as a basis for the implementation of visual modelling and analysis tools. The goal is to facilitate the specification, analysis and simulation of complex systems, using port graphs. A system is represented by an initial graph and a collection of graph rewriting rules, together with a user-defined strategy to control the application of rules. The strategy language includes constructs to deal with graph traversal and management of rewriting positions in the graph. We give a small-step operational semantics for the language, and describe its implementation in the graph transformation and visualisation tool PORGY.

==> eptcsdata.tex <==
\providecommand{\firstpage}{15}
\providecommand{\publicationstatus}{Dragan Bo\v{s}na\v{c}ki, Stefan Edelkamp, Alberto Lluch Lafuente\\ \& Anton Wijs (Eds.): 3rd Workshop on\\ GRAPH Inspection and Traversal Engineering (GRAPHITE 2014)\\
EPTCS 159, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.159.3}{10.4204/EPTCS.159.3}}
\pdfoutput=1

